Computational Polarization: An Information-theoretic Method for Resilient Computing

We introduce an error resilient distributed computing method based on an extension of the channel polarization phenomenon to distributed algorithms. The method leverages an algorithmic split operation that transforms two identical compute nodes to slow and fast workers, which parallels the channel split operation in Polar Codes. This operation preserves the average runtime, analogous to the conservation of Shannon capacity in channel polarization. By leveraging a recursive construction in a similar spirit to the Fast Fourier Transform, this method synthesizes virtual compute nodes with dispersed return time distributions, which we call computational polarization. We show that the runtime distributions form a functional martingale processes, identify their limiting distributions in closed-form expressions together with non-asymptotic convergence rates, and prove strong convergence results in Banach spaces. We provide an information-theoretic lower bound on the overall runtime of any coded computation method and show that the computational polarization approach asymptotically achieves the optimal runtime for computing linear functions. An important advantage is the near linear time decoding procedure, which is significantly cheaper than Maximum Distance Separable codes.

==> contents.tex <==
\section{Contents}
\begin{enumerate}
\item Abstract (9) 2
\item Introduction (20)
\item Overview (20)
\item Related work (30)
\item Preliminaries
	\begin{enumerate}
	\item Uncoded runtime
	\item MDS coded runtime
	\item Polar codes
	\end{enumerate}
\item Computational Polarization
	\begin{enumerate}
	\item Single Step
	\item Recursive
	\item Partial Polarization
	\end{enumerate}
\item Decoding
\item Heterogeneous computing 
\item Experimental results
	\begin{enumerate}
	\item Empirical CDFs
	\item Decoding times
	\item Matrix multiplication
	\item Gradient descent
	\end{enumerate}
\end{enumerate}
\if 0
convergence
limiting density
convergence rate
channel selection - different metrics polynomial martingale
joint density evolution
\fi


























==> discrete.tex <==
\subsection{Polarization of Discrete Distributions}
\begin{align*}
\left[\begin{array}{c}
p_1\\
p_2\\
\end{array} 
\right] 
\rightarrow 
\left[\begin{array}{c}
p^2_1\\
1-p_1^2\\
\end{array} 
\right]
,
\left[\begin{array}{c}
1-p^2_2\\
p^2_2\\
\end{array} 
\right]
\end{align*}



\begin{align*}
\left[\begin{array}{c}
p_1\\
p_2\\
p_3
\end{array}
\right]
\end{align*}
Corresponding CDF takes values $[1, 1-p_1, 1-p_1-p_2]$, first child will have values $[1, (1-p_1)^2, (1-p_1-p_2)^2]$, second child will have values $[1, 1-p_1^2, 1-(p_1+p_2)^2]$.

==> radonmeasures_old.tex <==
\subsection{Radon measures}
In this section, we briefly introduce mathematical background on Radon measures to state our main results. Consider a continuous function $f$ on the real line with scalar values. We say that $f$ has compact support if there is a bounded interval $[a,b]\subseteq \real$ such that $f(t)\neq 0$ implies that $0\le t\le b$. Let $\mathcal{C}_c$ denote the vector space of continuous scalar valued functions on $\real$ with compact support. A Radon measure is a positivity preserving linear functional $\mu$ from $\mathcal{C}_c$ to $\real$. The positivity preserving condition requires that
\begin{align*}
f(t)\ge 0\, \forall t \implies \langle \mu, f \rangle  \ge 0\,.
\end{align*}
We can construct Radon measures directly from cumulative distribution functions. Let $F$ be a right-continuous and non-decreasing function with support $[a,b]\subseteq \real$. We define the generalized inverse distribution function $G$ as
\begin{align*}
G(u) = \sup_{t\,:\, F(t) < u}{t}\,.
\end{align*}
Next, we define the Radon measure $\mu$ as
\begin{align*}
\langle \mu, f\rangle = \int_{a}^b f(G(u))du\,.
\end{align*}
Here, the preceding Lebesgue-Stieltjes integral can also be written as
\begin{align*}
\langle \mu, f\rangle = \int_{-\infty}^{\infty} f(t) dF(t)\,.
\end{align*}
Let us define the Dirac delta measure $\delta_{a}$ as the Radon measure which satisfies
\begin{align*}
\langle \delta_a, f \rangle = f(a)\,.
\end{align*}
It can be verified that $\delta_{a}$ is generated by the cumulative distribution function%
\begin{align*}
F(t) = \begin{cases} 0 \quad \mbox{ for } \quad t<a \\ 
1 \quad \mbox{ for } \quad t\ge a\,.
\end{cases}
\end{align*}
The corresponding inverse distribution function is given by
5
\begin{align*}
G(u) = a \quad \mbox{for}\quad 0 \le u \le 1\,. 
\end{align*}
